An Efficiency Study for SPLADE Models

Latency and efficiency issues are often overlooked when evaluating IR models based on Pretrained Language Models (PLMs) in reason of multiple hardware and software testing scenarios. Nevertheless, efficiency is an important part of such systems and should not be overlooked. In this paper, we focus on improving the efficiency of the SPLADE model since it has achieved state-of-the-art zero-shot performance and competitive results on TREC collections. SPLADE efficiency can be controlled via a regularization factor, but solely controlling this regularization has been shown to not be efficient enough. In order to reduce the latency gap between SPLADE and traditional retrieval systems, we propose several techniques including L1 regularization for queries, a separation of document/query encoders, a FLOPS-regularized middle-training, and the use of faster query encoders. Our benchmark demonstrates that we can drastically improve the efficiency of these models while increasing the performance metrics on in-domain data. To our knowledge, {we propose the first neural models that, under the same computing constraints, \textit{achieve similar latency (less than 4ms difference) as traditional BM25}, while having \textit{similar performance (less than 10\% MRR@10 reduction)} as the state-of-the-art single-stage neural rankers on in-domain data}.

==> figures/baselines/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.7\columnwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/baselines/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.29\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{70px}{%
         \input{figures/baselines/legend.tex}}
}
     \end{subfigure}
      \caption{Latency comparison between retrieval-based improvements. $^\dagger$: queries without stop words.}
     \label{fig:improvements}
\end{figure}





==> figures/baselines/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend entries={\textsc{i) + ii) - Baseline} ,
                        \textsc{iii) - Separate encoders} ,
                        \textsc{iv) - L1 Regularization},
                        \textsc{v) - PLM with FLOPS},
                        %\textsc{vi) - BERT-tiny},
                        %\textsc{vi) - Splade-doc},
                        %\textsc{vi) - Splade-doc$^\dagger$},
                        \textsc{Latency DistilBERT},
                        %\textsc{Latency BERT-tiny},
                        % \textsc{SoTA - ColBERTv2~\cite{santhanam2021colbertv2}},
                        }]
        \addlegendimage{baselineplot}
        \addlegendimage{separateplot}   
        \addlegendimage{lplotc}
        \addlegendimage{plmplotc}   
%        \addlegendimage{tinybertplot}
%        \addlegendimage{spladedocplot}   
%        \addlegendimage{spladedocstoppedplot}
        \addlegendimage{dash dot, orange}   
%        \addlegendimage{dashed, blue}   
%        \addlegendimage{thick, black}
        \end{customlegend}
\end{tikzpicture}


==> figures/baselines/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel=Latency (PISA) in ms,
           ylabel=MRR@10,
           xmin=-1, xmax=128, ymin=0.35, ymax=0.40]
         \addplot[baselineplot] table {figures/rq1/pisa_results_2.txt};
         \addplot[separateplot] table {figures/rq1/pisa_results_3.txt};
         \addplot[lplotc] table {figures/rq1/pisa_results_4.txt};
         \addplot[plmplotc] table {figures/rq1/pisa_results_5.txt};
%         \addplot[tinybertplot] table {figures/rq1/pisa_results_6.txt};
%         \addplot[spladedocplot] table {figures/rq1/pisa_splade_doc.txt};
%         \addplot[spladedocstoppedplot] table {figures/rq1/pisa_splade_doc_stopped.txt};
        \draw[dash dot, orange] (45.3,0) -- (45.3,1);
%        \draw[dashed, blue] (0.7,0) -- (0.7,1);
%        \draw[thick, black] (0,0.397) -- (1000,0.397);
       \end{axis}
    \end{tikzpicture}


==> figures/rq1/figure_large.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[t]{0.4\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq1/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.19\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{70px}{%
         \input{figures/rq1/legend.tex}}
}
     \end{subfigure}
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq1/anserini.tex}
}
        \end{subfigure}
      \caption{Latency comparison between all proposed improvements. Left is PISA retrieval and right is Anserini retrieval. We chose to omit the baseline of SPLADEv2 as it made the graphs harder to read (2 seconds latency on Anserini and 265 on Pisa). $^\dagger$: stop words removed from queries.}
     \label{fig:rq1}
\end{figure*}





==> figures/rq1_no_colbert/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.7\columnwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq1_no_colbert/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.29\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{70px}{%
         \input{figures/rq1_no_colbert/legend.tex}}
}
     \end{subfigure}
      \caption{Latency comparison between all proposed improvements. $^\dagger$: queries without stop words.}
     \label{fig:rq1}
\end{figure}





==> figures/rq1_no_colbert/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend entries={\textsc{i) + ii) - Baseline} ,
                        \textsc{iii) - Separate encoders} ,
                        \textsc{iv) - L1 Regularization},
                        \textsc{v) - PLM with FLOPS},
                        \textsc{vi) - BERT-tiny},
                        \textsc{vi) - Splade-doc},
                        \textsc{vi) - Splade-doc$^\dagger$},
                        \textsc{Latency DistilBERT},
                        \textsc{Latency BERT-tiny},
                         %\textsc{SoTA - ColBERTv2~\cite{santhanam2021colbertv2}},
                        }]
        \addlegendimage{baselineplot}
        \addlegendimage{separateplot}   
        \addlegendimage{lplotc}
        \addlegendimage{plmplotc}   
        \addlegendimage{tinybertplot}
        \addlegendimage{spladedocplot}   
        \addlegendimage{spladedocstoppedplot}
        \addlegendimage{dash dot, orange}   
        \addlegendimage{dashed, blue}   
%        \addlegendimage{thick, black}
        \end{customlegend}
\end{tikzpicture}


==> figures/rq1_no_colbert/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel=Latency (PISA) in ms,
           ylabel=MRR@10,
           xmin=-1, xmax=128, ymin=0.35, ymax=0.40]
         \addplot[baselineplot] table {figures/rq1/pisa_results_2.txt};
         \addplot[separateplot] table {figures/rq1/pisa_results_3.txt};
         \addplot[lplotc] table {figures/rq1/pisa_results_4.txt};
         \addplot[plmplotc] table {figures/rq1/pisa_results_5.txt};
         \addplot[tinybertplot] table {figures/rq1/pisa_results_6.txt};
         \addplot[spladedocplot] table {figures/rq1/pisa_splade_doc.txt};
         \addplot[spladedocstoppedplot] table {figures/rq1/pisa_splade_doc_stopped.txt};
        \draw[dash dot, orange] (45.3,0) -- (45.3,1);
        \draw[dashed, blue] (0.7,0) -- (0.7,1);
%        \draw[thick, black] (0,0.397) -- (1000,0.397);
       \end{axis}
    \end{tikzpicture}


==> figures/rq2/figure_large.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[t]{0.4\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq2/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.19\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{40px}{%
         \input{figures/rq2/legend.tex}}
}
     \end{subfigure}
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq2/anserini.tex}
}
        \end{subfigure}
      \caption{Latency comparison between the best improvements and the SoTA in sparse retrieval. Left is using PISA and right is using Anserini. $^\dagger$: stop words removed from queries.}
     \label{fig:rq2}
\end{figure*}





==> figures/rq2_no_colbert/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.7\columnwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{figures/rq2_no_colbert/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.29\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{50px}{%
         \input{figures/rq2_no_colbert/legend.tex}}
}
     \end{subfigure}
      \caption{Latency comparison between the proposed adaptations and sparse methods. $^\dagger$: queries without stop words.}
     \label{fig:rq2}
\end{figure}





==> figures/rq2_no_colbert/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend entries={\textsc{v) - PLM with FLOPS},
                        \textsc{vi) - BERT-tiny},
                        \textsc{vi) - Splade-doc$^\dagger$},
                        \textsc{BM25},
                        \textsc{BM25$^\dagger$},
                        \textsc{DocT5~\cite{doct5}},
                        \textsc{DeepImpact~\cite{10.1145/3404835.3463030}},
                        \textsc{uniCOIL-Tilde~\cite{zhuang2021fast}},
                        \textsc{Latency distilbert},
                         \textsc{Latency BERT-tiny},
                         %\textsc{SoTA - ColBERTv2~\cite{santhanam2021colbertv2}},
                        }]
        \addlegendimage{plmplotc}   
        \addlegendimage{tinybertplot}
        \addlegendimage{spladedocstoppedplot}
         \addlegendimage{bmvinplot};
         \addlegendimage{bmvinstoplot};
         \addlegendimage{docTplot};
         \addlegendimage{deepimpacplot};
         \addlegendimage{unicoilplot};
        \addlegendimage{dash dot, orange}   
        \addlegendimage{dashed, blue}   
%        \addlegendimage{thick, black}
        \end{customlegend}
\end{tikzpicture}


==> figures/rq2_no_colbert/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel=Latency (PISA) in ms,
           ylabel=MRR@10,
           xmin=-1, xmax=80, ymin=0.15, ymax=0.42,
           ]
         \addplot[plmplotc] table {figures/rq1/pisa_results_5.txt};
         \addplot[tinybertplot] table {figures/rq1/pisa_results_6.txt};
         \addplot[spladedocstoppedplot] table {figures/rq1/pisa_splade_doc_stopped.txt};
         \addplot[bmvinplot] table {figures/rq2/pisa_bm25.txt};
         \addplot[bmvinstoplot] table {figures/rq2/pisa_bm25_stopped.txt};
         \addplot[docTplot] table {figures/rq2/pisa_docT5.txt};
         \addplot[deepimpacplot] table {figures/rq2/pisa_deepimpact.txt};
         \addplot[unicoilplot] table {figures/rq2/pisa_unicoil-tilde.txt};
         
        \draw[dash dot, orange] (45.3,0) -- (45.3,1);
        \draw[dashed, blue] (0.7,0) -- (0.7,1);
%        \draw[thick, black] (0,0.397) -- (1000,0.397);
       \end{axis}
    \end{tikzpicture}

